In Shift and In Variance: Assessing the Robustness of HAR Deep Learning Models against Variability

Human Activity Recognition (HAR) using wearable inertial measurement unit (IMU) sensors can revolutionize healthcare by enabling continual health monitoring, disease prediction, and routine recognition. Despite the high accuracy of Deep Learning (DL) HAR models, their robustness to real-world variabilities remains untested, as they have primarily been trained and tested on limited lab-confined data. In this study, we isolate subject, device, position, and orientation variability to determine their effect on DL HAR models and assess the robustness of these models in real-world conditions. We evaluated the DL HAR models using the HARVAR and REALDISP datasets, providing a comprehensive discussion on the impact of variability on data distribution shifts and changes in model performance. Our experiments measured shifts in data distribution using Maximum Mean Discrepancy (MMD) and observed DL model performance drops due to variability. We concur that studied variabilities affect DL HAR models differently, and there is an inverse relationship between data distribution shifts and model performance. The compounding effect of variability was analyzed, and the implications of variabilities in real-world scenarios were highlighted. MMD proved an effective metric for calculating data distribution shifts and explained the drop in performance due to variabilities in HARVAR and REALDISP datasets. Combining our understanding of variability with evaluating its effects will facilitate the development of more robust DL HAR models and optimal training techniques. Allowing Future models to not only be assessed based on their maximum F1 score but also on their ability to generalize effectively

==> Tables/F1_Result.tex <==
\def\fscore#1{%
    \ifdim#1 pt>35pt
        \expandafter\cellcolor\expandafter{black!\number\numexpr 100 * #1 / 100}\color{white}%
    \else
        \expandafter\cellcolor\expandafter{black!\number\numexpr 100 * #1 / 100}\color{black}\fi#1
}
\begin{table}[!ht]
    \centering
    {
    \setlength\tabcolsep{3pt}%
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
        \textbf{Config} & \textbf{Model} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{C4} & \textbf{C5} & \textbf{C6} & \textbf{C7} & \textbf{C8} & \textbf{C9} & \textbf{C10} & \textbf{C11} & \textbf{C12} & \textbf{C13} & \textbf{C14} & \textbf{C15} & \textbf{C16} \\ \hline
        ER-EL & A\&D & \fscore{92} & \fscore{45} & \fscore{95} & \fscore{39} & \fscore{93} & \fscore{90} & \fscore{88} & \fscore{78} & \fscore{40} & \fscore{81} & \fscore{73} &\fscore {
    76} & \fscore{89} & \fscore{91} & \fscore{97} & \fscore{55} \\ \hline
         & DCL & \fscore{95} & \fscore{45} & \fscore{96} & \fscore{39} & \fscore{94} & \fscore{96} & \fscore{77} & \fscore{85} & \fscore{40} & \fscore{80} & \fscore{97} &\fscore {
            91} & \fscore{97} & \fscore{98} & \fscore{98} & \fscore{84} \\ \hline
         & THAR & \fscore{92} & \fscore{45} & \fscore{96} & \fscore{40} & \fscore{94} & \fscore{92} & \fscore{97} & \fscore{95} & \fscore{40} & \fscore{90} & \fscore{99} &\fscore {
            98} & \fscore{99} & \fscore{98} & \fscore{99} & \fscore{98} \\ \hline
        EL-EL & A\&D & \fscore{88} & \fscore{45} & \fscore{84} & \fscore{41} & \fscore{78} & \fscore{98} & \fscore{99} & \fscore{98} & \fscore{40} & \fscore{98} & \fscore{99} &\fscore {
    96} & \fscore{99} & \fscore{97} & \fscore{99} & \fscore{99} \\ \hline
         & DCL & \fscore{91} & \fscore{45} & \fscore{69} & \fscore{40} & \fscore{93} & \fscore{98} & \fscore{99} & \fscore{98} & \fscore{40} & \fscore{99} & \fscore{99} &\fscore {
            99} & \fscore{99} & \fscore{99} & \fscore{99} & \fscore{96} \\ \hline
         & THAR & \fscore{91} & \fscore{45} & \fscore{77} & \fscore{41} & \fscore{87} & \fscore{96} & \fscore{99} & \fscore{98} & \fscore{40} & \fscore{99} & \fscore{99} &\fscore {
            98} & \fscore{96} & \fscore{98} & \fscore{99} & \fscore{91} \\ \hline
        EL-ER & A\&D & \fscore{97} & \fscore{45} & \fscore{96} & \fscore{40} & \fscore{95} & \fscore{76} & \fscore{90} & \fscore{78} & \fscore{40} & \fscore{92} & \fscore{95} &\fscore {
    98} & \fscore{74} & \fscore{74} & \fscore{88} & \fscore{99} \\ \hline
         & DCL & \fscore{95} & \fscore{45} & \fscore{96} & \fscore{40} & \fscore{95} & \fscore{59} & \fscore{97} & \fscore{63} & \fscore{40} & \fscore{76} & \fscore{74} &\fscore {
            98} & \fscore{68} & \fscore{86} & \fscore{97} & \fscore{50} \\ \hline
         & THAR & \fscore{96} & \fscore{45} & \fscore{95} & \fscore{51} & \fscore{95} & \fscore{68} & \fscore{96} & \fscore{73} & \fscore{40} & \fscore{95} & \fscore{92} &\fscore {
            98} & \fscore{87} & \fscore{78} & \fscore{99} & \fscore{95} \\ \hline
        ER-ER & A\&D & \fscore{97} & \fscore{45} & \fscore{91} & \fscore{41} & \fscore{86} & \fscore{96} & \fscore{99} & \fscore{97} & \fscore{39} & \fscore{99} & \fscore{99} &\fscore {
    89} & \fscore{88} & \fscore{99} & \fscore{99} & \fscore{99} \\ \hline
         & DCL & \fscore{95} & \fscore{45} & \fscore{95} & \fscore{41} & \fscore{89} & \fscore{98} & \fscore{99} & \fscore{97} & \fscore{40} & \fscore{99} & \fscore{99} &\fscore {
            96} & \fscore{98} & \fscore{99} & \fscore{99} & \fscore{99} \\ \hline
         & THAR & \fscore{92} & \fscore{45} & \fscore{96} & \fscore{41} & \fscore{91} & \fscore{97} & \fscore{99} & \fscore{98} & \fscore{39} & \fscore{99} & \fscore{99} &\fscore {
            87} & \fscore{99} & \fscore{99} & \fscore{99} & \fscore{99} \\ \hline
        BL-EL & A\&D & \fscore{87} & \fscore{43} & \fscore{94} & \fscore{79} & \fscore{91} & \fscore{43} & \fscore{38} & \fscore{39} & \fscore{44} & \fscore{46} & \fscore{38} &\fscore {
    39} & \fscore{40} & \fscore{40} & \fscore{40} & \fscore{40} \\ \hline
        & DCL & \fscore{93} & \fscore{44} & \fscore{80} & \fscore{39} & \fscore{86} & \fscore{57} & \fscore{40} & \fscore{40} & \fscore{41} & \fscore{56} & \fscore{56} &\fscore {
            39} & \fscore{40} & \fscore{40} & \fscore{46} & \fscore{40} \\ \hline
         & THAR & \fscore{89} & \fscore{44} & \fscore{96} & \fscore{40} & \fscore{95} & \fscore{52} & \fscore{40} & \fscore{40} & \fscore{44} & \fscore{63} & \fscore{40} &\fscore {
            93} & \fscore{59} & \fscore{78} & \fscore{40} & \fscore{40} \\ \hline
        EL-BL & A\&D & \fscore{77} & \fscore{44} & \fscore{89} & \fscore{66} & \fscore{83} & \fscore{92} & \fscore{90} & \fscore{88} & \fscore{40} & \fscore{94} & \fscore{96} &\fscore {
    98} & \fscore{84} & \fscore{71} & \fscore{96} & \fscore{97} \\ \hline
        & DCL & \fscore{84} & \fscore{44} & \fscore{82} & \fscore{69} & \fscore{62} & \fscore{64} & \fscore{92} & \fscore{80} & \fscore{40} & \fscore{61} & \fscore{60} &\fscore {
            96} & \fscore{64} & \fscore{65} & \fscore{91} & \fscore{49} \\ \hline
         & THAR & \fscore{94} & \fscore{53} & \fscore{87} & \fscore{77} & \fscore{79} & \fscore{88} & \fscore{95} & \fscore{90} & \fscore{45} & \fscore{90} & \fscore{88} &\fscore {
            97} & \fscore{75} & \fscore{80} & \fscore{98} & \fscore{96} \\ \hline
        BL-BL & A\&D & \fscore{97} & \fscore{45} & \fscore{95} & \fscore{41} & \fscore{94} & \fscore{98} & \fscore{99} & \fscore{96} & \fscore{40} & \fscore{97} & \fscore{99} &\fscore {
    98} & \fscore{99} & \fscore{99} & \fscore{98} & \fscore{99} \\ \hline
         & DCL & \fscore{93} & \fscore{45} & \fscore{96} & \fscore{41} & \fscore{92} & \fscore{98} & \fscore{99} & \fscore{98} & \fscore{40} & \fscore{99} & \fscore{99} &\fscore {
            99} & \fscore{99} & \fscore{99} & \fscore{97} & \fscore{99} \\ \hline
         & THAR & \fscore{97} & \fscore{45} & \fscore{96} & \fscore{42} & \fscore{92} & \fscore{98} & \fscore{99} & \fscore{98} & \fscore{47} & \fscore{99} & \fscore{99} &\fscore {
            97} & \fscore{99} & \fscore{99} & \fscore{95} & \fscore{99} \\ \hline
        BR2-BR1 & A\&D & \fscore{84} & \fscore{45} & \fscore{91} & \fscore{41} & - & \fscore{98} & \fscore{93} & \fscore{98} & \fscore{39} & \fscore{91} & \fscore{98} &\fscore {
    98} & \fscore{99} & \fscore{98} & \fscore{99} & - \\ \hline
         & DCL & \fscore{76} & \fscore{45} & \fscore{90} & \fscore{41} & - & \fscore{97} & \fscore{99} & \fscore{95} & \fscore{42} & \fscore{92} & \fscore{94} &\fscore {
            96} & \fscore{98} & \fscore{98} & \fscore{98} & - \\ \hline
         & THAR & \fscore{90} & \fscore{45} & \fscore{95} & \fscore{45} & - & \fscore{98} & \fscore{97} & \fscore{98} & \fscore{39} & \fscore{93} & \fscore{99} &\fscore {
            98} & \fscore{96} & \fscore{97} & \fscore{99} & - \\ \hline
        BR1-BR1 & A\&D & \fscore{96} & \fscore{45} & \fscore{96} & \fscore{42} & - & \fscore{95} & \fscore{99} & \fscore{98} & \fscore{40} & \fscore{97} & \fscore{99} &\fscore {
    95} & \fscore{92} & \fscore{99} & \fscore{99} & - \\ \hline
         & DCL & \fscore{96} & \fscore{45} & \fscore{96} & \fscore{53} & - & \fscore{88} & \fscore{99} & \fscore{98} & \fscore{43} & \fscore{98} & \fscore{99} &\fscore {
            98} & \fscore{99} & \fscore{99} & \fscore{99} & - \\ \hline
        & THAR & \fscore{95} & \fscore{45} & \fscore{97} & \fscore{42} & - & \fscore{94} & \fscore{99} & \fscore{98} & \fscore{40} & \fscore{97} & \fscore{99} &\fscore {
            97} & \fscore{95} & \fscore{99} & \fscore{99} & - \\ \hline
        BR1-BR2 & A\&D & \fscore{58} & \fscore{44} & \fscore{91} & \fscore{50} & \fscore{70} & \fscore{69} & \fscore{97} & \fscore{94} & \fscore{40} & \fscore{92} &\fscore {
    97} & \fscore{87} & \fscore{59} & \fscore{96} & \fscore{98} & \fscore{39} \\ \hline
         & DCL & \fscore{91} & \fscore{44} & \fscore{91} & \fscore{73} & \fscore{90} & \fscore{76} & \fscore{98} & \fscore{79} & \fscore{50} & \fscore{96} & \fscore{89} &\fscore {
            87} & \fscore{76} & \fscore{98} & \fscore{98} & \fscore{39} \\ \hline
        & THAR & \fscore{44} & \fscore{44} & \fscore{97} & \fscore{47} & \fscore{88} & \fscore{92} & \fscore{97} & \fscore{91} & \fscore{46} & \fscore{89} &\fscore {
            72} & \fscore{98} & \fscore{38} & \fscore{94} & \fscore{98} & \fscore{38} \\ \hline
        BR2-BR2 & A\&D & \fscore{94} & \fscore{45} & \fscore{91} & \fscore{44} & \fscore{88} & \fscore{99} & \fscore{99} & \fscore{98} & \fscore{48} & \fscore{99} &\fscore {
    99} & \fscore{98} & \fscore{96} & \fscore{99} & \fscore{99} & \fscore{79} \\ \hline
         & DCL & \fscore{73} & \fscore{45} & \fscore{95} & \fscore{48} & \fscore{94} & \fscore{99} & \fscore{98} & \fscore{97} & \fscore{58} & \fscore{99} & \fscore{99} &\fscore {
            97} & \fscore{97} & \fscore{99} & \fscore{99} & \fscore{98} \\ \hline
         & THAR & \fscore{95} & \fscore{45} & \fscore{91} & \fscore{54} & \fscore{94} & \fscore{98} & \fscore{99} & \fscore{98} & \fscore{57} & \fscore{98} &\fscore {
            99} & \fscore{98} & \fscore{97} & \fscore{99} & \fscore{99} & \fscore{88} \\ \hline
        BR1-BL & A\&D & \fscore{38} & \fscore{38} & \fscore{44} & \fscore{56} & \fscore{41} & \fscore{74} & \fscore{35} & \fscore{40} & \fscore{56} & \fscore{40} & \fscore{37} &\fscore {
    40} & \fscore{39} & \fscore{40} & \fscore{33} & \fscore{40} \\ \hline
         & DCL & \fscore{43} & \fscore{48} & \fscore{48} & \fscore{42} & \fscore{39} & \fscore{86} & \fscore{41} & \fscore{43} & \fscore{56} & \fscore{40} & \fscore{39} &\fscore {
            40} & \fscore{40} & \fscore{40} & \fscore{40} & \fscore{40} \\ \hline
         & THAR & \fscore{42} & \fscore{44} & \fscore{44} & \fscore{56} & \fscore{37} & \fscore{40} & \fscore{40} & \fscore{40} & \fscore{59} & \fscore{40} & \fscore{39} &\fscore {
            40} & \fscore{40} & \fscore{41} & \fscore{40} & \fscore{40} \\ \hline
        BL-BR1 & A\&D & \fscore{42} & \fscore{41} & \fscore{27} & \fscore{41} & - & \fscore{37} & \fscore{40} & \fscore{40} & \fscore{59} & \fscore{47} & \fscore{37} &\fscore {
    36} & \fscore{40} & \fscore{32} & \fscore{40} & - \\ \hline
         & DCL & \fscore{42} & \fscore{45} & \fscore{42} & \fscore{72} & - & \fscore{57} & \fscore{40} & \fscore{40} & \fscore{56} & \fscore{44} & \fscore{41} &\fscore {
            40} & \fscore{53} & \fscore{42} & \fscore{71} & - \\ \hline
         & THAR & \fscore{50} & \fscore{43} & \fscore{42} & \fscore{63} & - & \fscore{46} & \fscore{40} & \fscore{40} & \fscore{48} & \fscore{58} & \fscore{39} &\fscore {
            67} & \fscore{40} & \fscore{40} & \fscore{40} & - \\ \hline
    \end{tabular}
    }
    \label{f1_all}
    \caption{The f1 score for all configurations using the HARVAR dataset. Configurations are shown in the Config column, representing the train and test pair. For example, ER-EL means that the model was trained using the empatica-right sensor and tested using the empatica-left sensor. C1-C16 are cross-validations per participant. Any cross-validation marked as "-" represents missing test data for the participant.}
\end{table}

==> Tables/MMD_Results.tex <==
\def\cca#1{%
    \ifdim#1 pt>35pt
        \expandafter\cellcolor\expandafter{black!\number\numexpr 100 * #1 / 70}\color{white}%
    \else
        \expandafter\cellcolor\expandafter{black!\number\numexpr 100 * #1 / 70}\color{black}\fi#1
}
\begin{table}[!ht]
    \centering
    {
    \setlength\tabcolsep{3pt}%
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
    \textbf{Config} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{C4} & \textbf{C5} & \textbf{C6} & \textbf{C7} & \textbf{C8} & \textbf{C9} & \textbf{C10} & \textbf{C11} & \textbf{C12} & \textbf{C13} & \textbf{C14} & \textbf{C15} & \textbf{C16} \\ \hline
        ER-EL & \cca{32} & \cca{64} & \cca{31} & \cca{43} & \cca{35} & \cca{45} & \cca{48} & \cca{47} & \cca{60} & \cca{46} & \cca{49} & \cca{47} & \cca{45} & \cca{47} & \cca{47} & \cca{49} \\ \hline
        EL-EL & \cca{57} & \cca{68} & \cca{52} & \cca{59} & \cca{51} & \cca{27} & \cca{27} & \cca{26} & \cca{61} & \cca{29} & \cca{28} & \cca{27} & \cca{27} & \cca{27} & \cca{25} & \cca{31} \\ \hline
        EL-ER & \cca{29} & \cca{66} & \cca{31} & \cca{44} & \cca{34} & \cca{43} & \cca{49} & \cca{48} & \cca{61} & \cca{44} & \cca{51} & \cca{49} & \cca{48} & \cca{47} & \cca{48} & \cca{46} \\ \hline
        ER-ER & \cca{54} & \cca{68} & \cca{51} & \cca{59} & \cca{47} & \cca{27} & \cca{27} & \cca{26} & \cca{62} & \cca{26} & \cca{27} & \cca{29} & \cca{30} & \cca{26} & \cca{26} & \cca{26} \\ \hline
        BL-EL & \cca{30} & \cca{65} & \cca{30} & \cca{47} & \cca{32} & \cca{46} & \cca{51} & \cca{50} & \cca{60} & \cca{46} & \cca{51} & \cca{50} & \cca{49} & \cca{49} & \cca{50} & \cca{52} \\ \hline
        EL-BL & \cca{51} & \cca{56} & \cca{47} & \cca{49} & \cca{47} & \cca{44} & \cca{45} & \cca{48} & \cca{51} & \cca{44} & \cca{47} & \cca{49} & \cca{44} & \cca{45} & \cca{47} & \cca{47} \\ \hline
        BL-BL & \cca{17} & \cca{61} & \cca{17} & \cca{33} & \cca{21} & \cca{20} & \cca{15} & \cca{17} & \cca{51} & \cca{18} & \cca{16} & \cca{18} & \cca{16} & \cca{14} & \cca{18} & \cca{17} \\ \hline
        BR2-BR1 & \cca{26} & \cca{62} & \cca{28} & \cca{35} & - & \cca{22} & \cca{29} & \cca{24} & \cca{55} & \cca{26} & \cca{24} & \cca{24} & \cca{19} & \cca{23} & \cca{23} & - \\ \hline
        BR1-BR1 & \cca{28} & \cca{64} & \cca{20} & \cca{33} & - & \cca{20} & \cca{24} & \cca{19} & \cca{54} & \cca{19} & \cca{18} & \cca{19} & \cca{20} & \cca{16} & \cca{17} & - \\ \hline
        BR1-BR2 & \cca{33} & \cca{66} & \cca{18} & \cca{34} & \cca{27} & \cca{22} & \cca{29} & \cca{25} & \cca{51} & \cca{20} & \cca{25} & \cca{21} & \cca{28} & \cca{19} & \cca{19} & \cca{40} \\ \hline
        BR2-BR2 & \cca{25} & \cca{65} & \cca{20} & \cca{35} & \cca{26} & \cca{20} & \cca{25} & \cca{19} & \cca{52} & \cca{21} & \cca{18} & \cca{20} & \cca{19} & \cca{17} & \cca{17} & \cca{32} \\ \hline
        BR1-BL & \cca{54} & \cca{54} & \cca{51} & \cca{48} & \cca{50} & \cca{47} & \cca{50} & \cca{52} & \cca{46} & \cca{48} & \cca{52} & \cca{54} & \cca{49} & \cca{50} & \cca{51} & \cca{52} \\ \hline
        BL-BR1 & \cca{53} & \cca{63} & \cca{51} & \cca{52} & - & \cca{45} & \cca{47} & \cca{49} & \cca{57} & \cca{47} & \cca{50} & \cca{50} & \cca{48} & \cca{49} & \cca{49} & - \\ \hline
    \end{tabular}
    }
    \label{mmd_all}
    \caption{The f1 score for all configurations using the HARVAR dataset. Configurations are shown in the Config column, representing the train and test pair. For example, ER-EL means that the model was trained using the empatica-right sensor and tested using the empatica-left sensor. C1-C16 are cross-validations per participant. Any cross-validation marked as "-" represents missing test data for the participant.}
\end{table}
